Characterizing the risk of fairwashing

Fairwashing refers to the risk that an unfair black-box model can be explained by a fairer model through post-hoc explanation manipulation. In this paper, we investigate the capability of fairwashing attacks by analyzing their fidelity-unfairness trade-offs. In particular, we show that fairwashed explanation models can generalize beyond the suing group (i.e., data points that are being explained), meaning that a fairwashed explainer can be used to rationalize subsequent unfair decisions of a black-box model. We also demonstrate that fairwashing attacks can transfer across black-box models, meaning that other black-box models can perform fairwashing without explicitly using their predictions. This generalization and transferability of fairwashing attacks imply that their detection will be difficult in practice. Finally, we propose an approach to quantify the risk of fairwashing, which is based on the computation of the range of the unfairness of high-fidelity explainers.

==> algos/fair_corels.tex <==
\begin{algorithm}
\caption{\faircorels{}}
\label{alg:faircorels}
\begin{algorithmic}[1]
\STATE Inputs: $X$, $Y$, $S$, $\epsilon$, 
$\unfair{}(r, X, Y)$, 
$\obj{}(r, X, Y)$, 
$\lwb{}(r, X, Y)$, 
$(\arule^0, \aruleobj^0)$ 
\STATE Output: $\arule^*$ 
\STATE $(\arule^c, \aruleobj^c) \gets  (\arule^0, \aruleobj^0)$
\STATE $Q \gets queue([()])$ 
\WHILE{$Q$ not empty}
    \STATE $\arule \gets Q.pop()$ 
    \IF{$\lwb{}(\arule, X, Y) < \aruleobj^c$}            
        \STATE $\aruleobj{} \gets \obj{}(\arule, X, Y)$
        \STATE $u \gets \unfair{}(\arule, X, Y)$ 
        \IF{$\aruleobj{} < \aruleobj^c$ and $u \leq \epsilon$} 
            \STATE $(\arule^c, \aruleobj{}^c) \gets (\arule, \aruleobj)$ 
        \ENDIF
        \FOR {$s$ in $S$} 
            \IF{$s$ not in  $\arule$} 
                    \STATE $Q.push((\arule,s))$
            \ENDIF
        \ENDFOR
    \ENDIF
\ENDWHILE
\STATE $(\arule^*, \aruleobj^*) \gets  (\arule^c, \aruleobj^c)$
\end{algorithmic}
\end{algorithm}




==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{sec:exp1} for results related to the characterization of the \fidunf{} trade-offs in fairwashing, Section~\ref{sec:exp2} for results related to the generalization of fairwashing beyond suing groups and Section~\ref{sec:exp3} for results related to the transferability of fairwashing across black-box models.}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{All the code to reproduce all the experimental results is included in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We included the code of our experiments.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/explanations_manipulations.tex <==
\begin{table*}[htbp]
\centering
\caption{Summary of related work for the manipulation of post-hoc explanations.}
\label{tab:explainWashing}
\vskip 0.15in
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{Name of attack} & \multirow{2}{*}{Reference} & \multirow{2}{*}{Model agnostic attack} & Explanation type &  \\ \cmidrule(l){4-5} 
 &  &  & Global & Local \\ \midrule
Fairwashing & \cite{aivodji2019fairwashing} & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
Stealthily biased sampling & \cite{fukuchi2020faking} & $\checkmark$ & $\checkmark$ & $\times$ \\
%Misleading explanation maps & \begin{tabular}[c]{@{}c@{}}\cite{heo2019fooling}\\ \cite{dombrowski2019explanations}\\ \cite{anders2020fairwashing}\end{tabular} & $\times$ & $\times$ & $\checkmark$ \\
Misleading explanation maps & \cite{heo2019fooling} & $\times$ & $\times$ & $\checkmark$ \\
& \cite{dombrowski2019explanations} & $\times$ & $\times$ & $\checkmark$ \\
& \cite{anders2020fairwashing} & $\times$ & $\times$ & $\checkmark$ \\
Unjustified counterfactual explanations & \cite{laugel2019dangers} & $\checkmark$ & $\times$ & $\checkmark$ \\
Public relations attack & \cite{le2020remote} & $\checkmark$ & $\times$ & $\checkmark$ \\
Scaffolding & \cite{slack2019can} & $\checkmark$ & $\times$ & $\checkmark$ \\
Misleading black-box explanations & \cite{lakkaraju2020fool} & $\checkmark$ & $\checkmark$ & $\times$ \\ \bottomrule
\end{tabular}%
}
\end{table*}

==> tables/group_fairness_notions.tex <==
\begin{table*}[h!]
\caption{Summary of the different statistical notions of fairness considered.}
\label{tab:group_fairnes_notions}
\vskip 0.15in
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\hline
\textbf{Fairness notion} & \textbf{Definition} \\ \hline
Statistical Parity ($\sp{}$) & $|P(\hat{Y}=1|G=0) - P(\hat{Y}=1|G=1)|$ \\
Predictive Equality ($\pe{}$) & $|P(\hat{Y}=1|Y=0,G= 0) - P(\hat{Y}=1|Y=0,G= 1)|$ \\
Equal Opportunity ($\eop{}$) & $|P(\hat{Y}=1|Y=1,G= 0) - P(\hat{Y}=1|Y=1,G= 1)|$ \\
Equalized Odds ($\eodds{}$) & $|P(\hat{Y}=1|Y=1,G=0) - P(\hat{Y}=1|Y=1,G=1)|$ and  $|P(\hat{Y}=1|Y=0,G=0) - P(\hat{Y}=1|Y=0,G=1)|$ \\
\hline
\end{tabular}%
}
\end{table*}
